An Intentional Forgetting-Driven Self-Healing Method For Deep Reinforcement Learning Systems

Deep reinforcement learning (DRL) is increasingly applied in large-scale productions like Netflix and Facebook. As with most data-driven systems, DRL systems can exhibit undesirable behaviors due to environmental drifts, which often occur in constantly-changing production settings. Continual Learning (CL) is the inherent self-healing approach for adapting the DRL agent in response to the environment's conditions shifts. However, successive shifts of considerable magnitude may cause the production environment to drift from its original state. Recent studies have shown that these environmental drifts tend to drive CL into long, or even unsuccessful, healing cycles, which arise from inefficiencies such as catastrophic forgetting, warm-starting failure, and slow convergence. In this paper, we propose Dr. DRL, an effective self-healing approach for DRL systems that integrates a novel mechanism of intentional forgetting into vanilla CL to overcome its main issues. Dr. DRL deliberately erases the DRL system's minor behaviors to systematically prioritize the adaptation of the key problem-solving skills. Using well-established DRL algorithms, Dr. DRL is compared with vanilla CL on various drifted environments. Dr. DRL is able to reduce, on average, the healing time and fine-tuning episodes by, respectively, 18.74% and 17.72%. Dr. DRL successfully helps agents to adapt to 19.63% of drifted environments left unsolved by vanilla CL while maintaining and even enhancing by up to 45% the obtained rewards for drifted environments that are resolved by both approaches.

==> _evaluation_backup.tex <==
In this section, we first introduce the DRL case studies (environments and algorithms), as well as our experimental settings, metrics, and procedure. Next, we evaluate \name{} against vanilla CL in terms of cost reduction (RQ1), adaptability enhancement (RQ2), and reward improvement (RQ3).
\subsection{Experimental Setup}
\subsubsection{Environments}
We leverage the following 3 different environments in our empirical evaluation. \\
\textbf{The MountainCar environment} \cite{moore1990efficient} was described in the previous section (see Section \ref{sec:example}), along with the parameters we vary to simulate environment drift. \\
\textbf{The CartPole environment} \cite{barto1983neuronlike} is an inverted pendulum connected to a cart by an unactuated joint. The cart moves on a track, which is controlled by a force either pushing it to the right direction $(+1)$ or to the left ($-1$) with the same magnitude. Keeping the pole upright is the objective of moving the cart; so the agent gets $+1$ every time the pole stays upright. The task of controlling the cart is episodic, and the episode ends when the pole falls over $15^{\circ}$, the cart moves $2.4$ units from the center, or $200$ time steps pass. An agent is considered to have solved a task when their average reward over $100$ testing episodes is greater than $195$. The CartPole environment can be parameterized using four parameters: masspole, length pole, mass cart, and friction. \\
\textbf{The Acrobot environment} \cite{geramifard2015rlpy, sutton1995generalization} has two joints and two links where the joint between the two links can be actuated. Initial position of the system is with the links hanging downwards and the agent aims to raise the lower link to a given height. If the agent reaches its goal, it gets a reward of $0$; otherwise, it gets $-1$ at every timestep. Episodes in Acrobot environment end when the goal or $500$ time steps are reached. There is a reward threshold for the Acrobot environment that is $-100$ over $100$ evaluation episodes. The environment parameters include 'link length 1' (length of the first link), 'link compos 1' (position of the center of mass of the first link), 'link mass 1' and 'link mass 2' (mass of both links).
\subsubsection{DRL Algorithms}
In the following, we present the selected DRL algorithms for our evaluation. They are mature and widely used, and as such many model-free RL libraries provide a stable implementation of them. \\
\textbf{Deep Q-Learning (DQN)} \cite{mnih2015human} is a popular value-based method that has evolved over the years with a variety of optimizations \cite{urtans2018survey}. DQN leverages neural network to approximate the action-value function, Q. Iterative learning of Q does not guarantee convergence, instabilities leading to divergence can be addressed by two techniques: using a buffer to replay older experiences and using two DNNs to stabilize the learning process. DQN uses an $\epsilon$-greedy policy, where the agent selects the optimal action with probability $1 - \epsilon$, or a random action with probability $\epsilon$. Furthermore, $\epsilon$ is linearly annealed from $1.0$ to $0.1$ for $K$ steps. Hence, the agent explores much more in the early training phase, while exploitation occurs more at the end. \\
\textbf{Proximal Policy Optimization (PPO)} \cite{schulman2017proximal} is a state-of-the-art algorithm whose goal is to improve the policy as much as possible without compromising performance. For stable policy updates, PPO uses clipping mechanism to prevent too much change to the policy and a hyperparameter, $\epsilon$, that controls how much it can diverge from the last policy. Instead of learning from current experience and discarding past experiences, PPO is designed to reuse even old experiences, which makes it more sample efficient. PPO trains a stochastic policy that explores the environment in its initial phases of training, but gradually it becomes more deterministic and encourages the agent to exploit rather than explore.\\
\textbf{Soft Actor Critic (SAC)} \cite{haarnoja2018soft} focuses on maximizing returns and policy entropy (i.e. degree of its "randomness"), simultaneously. SAC also performs its updates off-policy, similar to DQN. More precisely, to encourage exploration, SAC regulates the entropy of the policy through a coefficient $\alpha$, which can be fixed manually or adjusted automatically over the training. In our tests, we use the auto-adjusted version of the entropy regularization coefficient $\alpha$.
\subsubsection{Software and Hardware Configuration}
We implemented our approach as an open-source tool using Python 3.7~\cite{van2009python} and it supports Tensorflow (version 2.4.4)~\citep{abadi_tensorflow}. We evaluated environments from the Gym library (version 0.23.1)~\cite{brockman2016openai} and DRL algorithms adapted from popular GitHub repositories \cite{noauthor_welcome_nodate, TF2RL}. We used two GPU-enabled servers. The first server runs Ubuntu 20.04 and features a 24-core AMD EPYC 7413 CPU, an ASPEED AST2500 GPU, and 500 GB of RAM. The second runs CentOS 7 and has a 12-core 1.70 GHz Intel Xeon Bronze CPU, an NVIDIA GeForce RTX 2080 Ti GPU.
\subsubsection{Evaluation Procedure and Metrics}\hfill\\
\noindent{\textbf{Procedure:}} The DRL algorithms' hyperparameters were tuned using the open-source repository rl-baselines-zoo~\citep{stable_baselines}, which offers information on the implementation and configuration of popular DRL algorithms. Given the current study's concerns that minor implementation details might substantially affect DRL algorithm performance~\citep{engstrom2020implementation}, we conducted ten distinct training runs with various random seeds to further tweak the DRL algorithms. The final hyperparameters for each DRL algorithm were chosen based on the highest average reward. Next, for each DRL algorithm we investigated, we sampled six environmental drift settings with realistic values. More specifically, we deliberately induce drifts of varying magnitudes to simulate different shifts that may occur in production. In fact, to discern between the intensities of the simulated drifts, we rely on the environment's parameter ranges described in the study of Biagiola and Tonella~\citep{tonella}. Then, we apply our approach, \name{}, and vanilla CL to adapt the agent to the six newly-drifted environments. To have a fair comparison, we used the same hyperparameters and max number of episodes of the DRL agent beforehand. Nevertheless, we tuned the specific parameters, $F_r$ and $S_r$, of \name{} for each environment using, respectively, the ranges of [50, 40, 30, 20, 10]\% and [0.00001, 0.0001, 0.001, 0.01, 0.1]. We found that the best parameters are $F_r$=50\% and $S_r$=0.1 for the CartePole environment. For both Acrobot and MountainCar environments, $F_r$=10\% and $S_r$=0.0001 work better. The difference in the parameters of \name{} can be explained by the level of difficulty . In this case, CartePole is the easiest environment to solve. The other two environments, MountainCar and Acrobot, are more challenging given their deceptive nature. In these deceptive reward environments, the agent is misled and discouraged from exploring (by offering a negative reward), causing it to fall into the local optimal stage. Moreover, following the logic of Biagiola and Tonella~\citep{tonella}, we assign an adaptability tolerance ratio of 20\% to these two environments. In other words, we introduce an accepted 20\% of performance degradation for these environments during adaptation. For instance, in the MountainCar environment, the agent adapts to the drifted environment if it gets an average reward of $-132$, corresponding to $-110$ (solved environments) minus 20\% (see Figure~\ref{fig:avg_reward}).\\
Finally, all experiments are run 10 times to overcome the stochastic nature of these DRL algorithms. We apply statistical significance tests to compare the results obtained by \name{} and plain CL. In particular, we use the non-parametric Wilcoxon~\citep{wilcoxon_individual_1945} test and the Vargha-Delaney A12 effect size~\citep{vargha2000critique}.\\
\textbf{Metrics:} Below, we introduce the different evaluation metrics that have been used in the empirical evaluations.\\ 
\textit{Increase Ratio (\%IR(X)) / Decrease Ratio (\%DR(X)).} It consists of the percentage increase/decrease of the quantity X from applying \name{} rather than CL, as formulated in Eq.~\ref{IR}/Eq.~\ref{DR}. Thereby, positive values indicate the on-watch quantity, X, improved whereas negative values indicate a degradation.\\
\begin{equation}
\label{IR}
\%IR(X) = \dfrac{\textit{\name{}\_X} - \textit{CL\_X}}{\textit{CL\_X}} \times 100
\end{equation}

\begin{equation}
\label{DR}
\%DR(X) = \dfrac{\textit{CL\_X} - \textit{\name{}\_X}}{\textit{CL\_X}} \times 100
\end{equation}

\rached{should we change the name of this metric ?}
\textit{Adaptability Ratio (\%AR).} It consists of the percentage of pairs (a trained DRL agent, a drifted environment) that a given approach Y is able to adapt, as formulated in Eq.~\ref{AR}.

\begin{equation}
\label{AR}
\%AR(Y) = \dfrac{ \textit{(Env, Agent)}_{adpt_{(Y)}}}{ \textit{(Env, Agent)}_{All}} \times 100
\end{equation}

\subsection{Research Questions and Answers}

% \subsubsection{RQ1: Is \name{}'s agent adaptation more cost-effective than continual learning ?} \hfill 

% \textbf{Motivation:}  The purpose is to compare \name{} with the vanilla CL technique in terms of the cost effectiveness of adapting the DRL trained agent in drifted environments. When an agent is fine-tuned to operate in a new environment, delayed convergence can result in substantial financial penalties, and a high number of trials makes it difficult to apply to physical robots.

% \noindent{\textbf{Method:}} In order to compare the cost-effectiveness, the amount of time and episodes necessary to adjust an agent to a drifted environment were measured using both methods, \name{} and CL. An episode ends when the agent has reached its goal or failed to reach it after completing the maximum number of steps allowed in each episode, which is dependent on the environment. Hence, we track how long the agent spends adjusting to the drifted environment and how many episodes it takes for the evaluated method to complete the adaptation. In order to meet the completion criteria, the agent must achieve a reward greater than the threshold set by the environment for 100 consecutive episodes (\ahmed{this is not consistent with figure 2, we mean average reward over 100 episodes!}). To have a better understanding of the magnitude of speed-up obtained when using \name{} compared to CL, we compute the decrease ratio, \%DR (Eq.~\ref{DR}), of both the training time and the training  episodes. 

% \begin{table}[]
%     \caption{Comparison of Adaptation Time and Fine-Tuning Episodes Decreases Using \name{} over CL.}
%     \label{tab:time}
%     \centering
%         \input{tables/time.tex}
% \end{table}

% \noindent{\textbf{Results:}} Table \ref{tab:time} reports the DRL agent's running time and number of episodes required to adapt its logic to the newly shifted environment using our approach, \name{}, and vanilla CL. The bold values indicate that the difference between the two compared entities is statistically significant (i.e., the p-value is below 0.05) and the underline indicates when the magnitude of the effect size A12 is medium or large.

% Overall, \name{} outperforms CL in terms of cost effectiveness. As can be seen, \name{} provides faster adaptation time for DRL agents than CL, except for the study case of PPO/CartePole. The difference between the two averaged values is statistically significant in $56\%$ of the evaluated configurations and of a substantial magnitude in $33\%$ of the configurations. In terms of fine-tuning episodes, \name{} uses fewer episodes to adapt the DRL agent to drifted environments than CL across all the pairs of agents and environments. Especially, \name{} adapts PPO to the drifted CartePole with very few episodes, meaning the overhead of execution time was caused by longer time steps. There is a significant difference between the two approaches in terms of training episodes in $44\%$ of the evaluated configurations. Also, the effect size of this difference is medium or large in these configurations.

% These results demonstrate the effectiveness of our approach, \name{}, in reducing sample complexity, i.e., the number of episodes of play, in order to determine the best policy. Investigating the sample complexity of RL algorithms has been a major focus of research studies~\cite{xie2021policy}, and enhancing the sample efficiency is crucial to expanding DRL-based systems in real-world applications.

% \begin{tcolorbox}[colback=blue!5,colframe=blue!40!black]
% \textbf{Finding 1.} \name{} provides a sample-efficient adaptation of DRL agents to drifted environments, resulting in fewer fine-tuning episodes and shorter runtime. 
% \end{tcolorbox}

% \subsubsection{RQ2: To what extent does \name{} enhance the plasticity/adaptability of DRL agents to drifted environments?} \hfill

% \textbf{Motivation:} The objective is to determine if \name{} can adapt an agent to drifted environments that cannot be resolved through continual learning, and vice versa.

% \noindent{\textbf{Method:}} To compare the plasticity of DRL agents resulting from different adaptation methods, we compute their adaptability ratios (\%AR). Then, we expect four possible scenarios: (1) agent-environment pairs handled by both adaptation methods; (2) pairs handled exclusively by \name{}; (3) pairs handled exclusively by vanilla continual learning; and (4) pairs not handled by both methods.

% \begin{figure*}[h]
% \centering
% \includegraphics[width=0.8\textwidth]{figures/pie.PNG}
% \caption{Distribution of Adaptable vs Non-Adaptable Cases Per Adaptation Method and RL Environment}
% \label{fig:pie_chart}
% \end{figure*}

% \noindent{\textbf{Results:}} Figure \ref{fig:pie_chart} shows (a) Pie chart showing the adaptability ratios achieved by either \name{}, vanilla continual learning, both, or none of them; (b) Pie charts depicting the results of adaptability ratios broken down by environment. 

% As can be seen in Figure \ref{fig:pie_chart}-a, our approach succeeds in adapting the majority of the agent-environment pairs on which vanilla continual learning succeeds as well. Indeed, the cases where \name{} fails against continual learning are very few, about 4\%. The reason is that any reduction of parameters, no matter how carefully screened or guided, induces a loss of information that may lead to inefficiencies in the DRL agent like diminished plasticity. Hence, our intentional forgetting mechanism improves the sample efficiency of continual learning without compromising the DRL agent plasticity in most of the cases.\\
% Interestingly, \name{} is able to adapt about 20\% of agent-environment pairs on which vanilla continual learning fails. This proves the utility of \name{} in the enhancement of the DRL agent plasticity against a subset of environmental drifts that were formerly considered non-adaptable cases, which results in extending the frontiers of continual learning.\\
% In line with the previous study on DRL agent plasticity, there is a substantial proportion of drifted environments that are beyond the capability of continual learning, including the vanilla version and the improved version of \name{}. This suggests that the continuous adaptation of pre-trained DRL agents to similar environments with constantly-shifting parameters has limits, and there are severe environmental drifts for which a redesign of the DRL agent or re-training from scratch can be more suitable to solve the problem.

% According to Figure \ref{fig:pie_chart}-b, the agent-environment pairs that are adapted exclusively by one of the two methods, \name{}, remain almost equal for the different studied environments. Meanwhile, the proportions of pairs that are either adapted or unadapted equally by both methods are correlated with the difficulty of the underlying environment. Therefore, although their differences are independent of the environment, both adaptation methods degrade in performance when exposed to challenging drifted environments, i.e., involving high dimensional and sensitive settings, leading to less successfully-adapted DRL agents as well as more non-adaptable ones.

% \begin{tcolorbox}[colback=blue!5,colframe=blue!40!black]
% \textbf{Finding 2.} \name{} outperforms the vanilla CL in adapting a higher proportion of DRL agents to drifted environments, thus expanding their plasticity frontiers.

% \end{tcolorbox}

% \subsubsection{RQ3: Are \name{}'s adapted agents more performant in terms of reward than their CL's counterparts ?} \hfill 

% \noindent{\textbf{Motivation:}} The goal is to compare \name{} with the continual learning strategy in regards to the achieved performance of the adapted agent on drifted environments. 

% \noindent{\textbf{Method:}} In this RQ, we consider the two following scenarios: (i) jointly adaptable environments, belonging to agent-environment pairs where CL and \name{} both succeeded in adapting the DRL agent; (ii) jointly non-adaptable environments, belonging to agent-environment pairs where CL and \name{} both failed in adapting the DRL agent. In these two scenarios, we average the rewards obtained by the adapted agent over the course of 100 consecutive episodes, using both alternative methods. Then, we calculate \name{}'s average reward increase ratio, \%IR (Eq.~\ref{IR}), w.r.t the CL's average reward. Besides, the remaining scenarios, in which one method succeeds and the other fails, are irrelevant for reward comparison because the gap between them will be wide due to the failure of adaptation.
% \begin{table}[]
%     \caption{Comparison of Adapted DRL Agent Reward Increases Using Dr.DRL over CL.}
%     \label{tab:reward}
%     \centering
%         \input{tables/reward.tex}
% \end{table}


% \noindent{\textbf{Results:}} The first part of Table \ref{tab:reward} (i.e., Rows 2–4) shows the reward increase ratio of \name{} compared to vanilla continual learning in jointly adaptable environments. \name{} achieves a similar average reward (no less than -1.2\%) compared to continual learning in 78\% of configurations. In the remaining 22\% of configurations, \name{} increases the average reward obtained by at least 10\%. To conclude, \name{} succeeds in preserving or improving the baseline average reward achieved by continual learning in jointly adapted environments.\\
% The second part of Table \ref{tab:reward} (Rows 5-7) shows the reward increase ratio of \name{} compared to vanilla continual learning in jointly non-adaptable environments. As can be seen, \name{} was able to improve the average reward in 78\% of the configurations by up to 45\% of increase ratio w.r.t CL's average reward. Hence, we highlight how \name{} achieves average rewards closer to the requirements compared to CL in the drifted environments that are still non-adaptable by both approaches.

% \begin{tcolorbox}[colback=blue!5,colframe=blue!40!black]
% \textbf{Finding 3:} \name{} was capable of achieving similar or even higher rewards in adaptable environments, and it also earned higher rewards in non-adaptable ones, showing how much closer \name{} was to meet the requirements than CL.
% \end{tcolorbox}

\subsubsection{RQ1 (Cost-effectiveness): How cost-effective \name{} is in adapting DRL systems compared to continual learning?} \hfill  

\textbf{Motivation:} The purpose is to compare \name{} with the vanilla CL technique in terms of the cost-effectiveness of healing the DRL systems in drifted environments. Fine-tuning DRL systems to operate in a new environment requires simulation and/or live deployment, which can be resource-intensive and costly. Consequently, delays in healing the behaviour of the DRL agent can result in substantial cost penalties, and the effectiveness of repair may be hindered by a high number of required trials in order to optimize the agent's behaviour.
% The purpose is to compare \name{} with the vanilla CL technique in terms of the cost-effectiveness of healing the DRL systems in drifted environments. Fine-tuning DRL systems to operate in a new environment requires simulation and/or live deployment, which can be pretty expensive and necessitates a significant investment in resources. Therefore, self-adaptation (or repair) delay can result in substantial cost penalties, and a high number of trials makes the repair difficult to apply.
\noindent{\textbf{Method:}} To compare the cost-effectiveness of \name{} and CL, we measured the amount of time and episodes necessary to heal a DRL system in a drifted environment. An episode ends when the agent has reached its goal or failed to reach it after completing the maximum number of steps allowed in each episode, which is determined by the specific environment. Hence, we track how long the agent spends adjusting to the drifted environment and the number of episodes needed for each of the evaluated strategy to heal the agent. To meet the completion criteria, the agent must achieve an average reward over 100 consecutive episodes greater or equal to the threshold set by the environment. To have a better understanding of the magnitude of speed-up obtained when using \name{} compared to CL, we compute the decrease ratio, \%DR (Eq.~\ref{DR}), of both the training time and the training episodes. 

% To compare the cost-effectiveness of \name{} and CL, we measured the amount of time and episodes necessary to heal a DRL system to a drifted environment. An episode ends when the agent has reached its goal or failed to reach it after completing the maximum number of steps allowed in each episode, which is dependent on the environment. Hence, we track how long the agent spends adjusting to the drifted environment and how many episodes it takes for the evaluated strategy to complete the adaptation. To meet the completion criteria, the agent must achieve an average reward over 100 consecutive episodes greater or equal to the threshold set by the environment. To have a better understanding of the magnitude of speed-up obtained when using \name{} compared to CL, we compute the decrease ratio, \%DR (Eq.~\ref{DR}), of both the training time and the training episodes. 
\begin{table}[]
    \caption{Comparison of Healing Time and Fine-Tuning Episodes Decreases Using \name{} over CL.}
    \label{tab:time}
    \centering
        \input{tables/time.tex}
\end{table}

\noindent{\textbf{Results:}} Table \ref{tab:time} reports the DRL system's running time and number of episodes required to adjust its logic to the newly shifted environment using our approach, \name{}, and vanilla CL. The bold values indicate that the difference between the two compared entities is statistically significant (i.e., the p-value is below $0.05$) and the underline indicates when the magnitude of the effect size A12 is medium or large.

Overall, \name{} outperforms CL in terms of cost-effectiveness. As can be seen, \name{} provides a faster healing time for DRL systems than CL, except for the study case of PPO/CartePole. The difference between the two averaged values is statistically significant in $56\%$ of the evaluated configurations and of a substantial magnitude in $33\%$ of the configurations. In terms of fine-tuning episodes, \name{} uses fewer episodes to adapt the DRL system to drifted environments than CL across all the pairs of agents and environments. Especially, \name{} adapts PPO to the drifted CartePole with very few episodes, meaning the overhead of execution time was caused by longer time steps. There is a significant difference between the two approaches in terms of training episodes in $44\%$ of the evaluated configurations. Also, the effect size of this difference is medium or large in these configurations.

These results demonstrate the effectiveness of our approach, \name{}, in lowering the cost of healing the agent's behaviour by reducing the sample complexity, i.e., the number of training episodes, in order to determine the best policy. Investigating the sample complexity of RL algorithms has been a major focus of research studies~\cite{xie2021policy}, and enhancing the sample efficiency is crucial to expanding DRL-based systems in real-world applications.

\begin{tcolorbox}[colback=blue!5,colframe=blue!40!black]
\textbf{Finding 1.} \name{} enables a cost-efficient healing of DRL systems in drifted environments, through fewer fine-tuning episodes and shorter healing time. 
\end{tcolorbox}

\rached{I dont think we should change adaptability here}
\subsubsection{RQ2 (healing frontiers): Can \name{} enhance the adaptability of DRL systems to drifted environments?} \hfill

\textbf{Motivation:} The objective is to determine if \name{} can heal a DRL system to drifted environments that cannot be resolved through CL and vice versa. It was recently demonstrated [ref] that the CL has an environmental boundary beyond which it cannot adjust the DRL system. \name{} was established with the intention of expanding this boundary.

\noindent{\textbf{Method:}} To compare the adaptation of DRL systems resulting from different healing strategies, we compute their adaptability ratios (\%AR) (Eq.~\ref{AR}). Then, we expect four possible scenarios: (1) agent-environment pairs fitted by both healing strategies (\name{} and vanilla CL); (2) pairs fitted exclusively by \name{}; (3) pairs fitted exclusively by vanilla CL; and (4) pairs not fitted by both strategies.

\begin{figure*}[h]
\centering
\includegraphics[width=0.8\textwidth]{figures/pie.PNG}
\caption{Distribution of Adaptable vs Non-Adaptable Cases Per healing Method and RL Environment}
\label{fig:pie_chart}
\end{figure*}

\noindent{\textbf{Results:}} Figure \ref{fig:pie_chart} shows (a) the Pie chart demonstrating the global adaptability ratios achieved by either \name{}, vanilla CL, both, or none of them; and (b) Pie charts depicting the results of adaptability ratios broken down by environments.

As can be seen in Figure \ref{fig:pie_chart}-a, our approach succeeds in adapting the majority of the agent-environment pairs on which vanilla CL succeeds as well. Indeed, the cases where \name{} fails against CL are very few, about 4\%. The reason is that any reduction of parameters (i.e., hypoactive neurons), no matter how carefully screened or guided, induces a loss of information that may lead to inefficiencies in the DRL system (e.g., diminished adaptability). The above demonstrates that in most circumstances, our intentional forgetting mechanism enhances the cost-efficiency (i.e., the sample efficiency) of CL (RQ1) without compromising DRL system adaptability.\\
Interestingly, \name{} is able to adapt about 20\% of agent-environment pairs on which vanilla CL fails. This proves the effectiveness of \name{} in the enhancement of the DRL system adaptability against a subset of previously deemed non-adaptable environmental drifts, which results in extending the frontiers of CL. As a result, \name{} not only preserves but also expands CL's adaptability frontiers, enhancing the DRL system's self-adaptability.\\
In line with the previous study on DRL system adaptability [ref], there is a substantial proportion of drifted environments that are beyond the capability of CL, including the vanilla version and the improved version of \name{}. This suggests that the continuous adaptation of pre-trained DRL agents to similar environments with constantly-shifting parameters has limits. Therefore, for some environmental drifts, the redesign of the DRL system or re-training from scratch can be more suitable to solve the problem.

According to Figure \ref{fig:pie_chart}-b, the proportions of agent-environment pairs that are adapted exclusively by one of the two strategies remain almost constant across the three studied environments. Meanwhile, the proportions of pairs that are either adapted or unadapted equally by both strategies are correlated with the difficulty of the underlying environment. Therefore, although their differences are independent of the environment, both adaptation strategies degrade in the adaptability performance when exposed to challenging drifted environments, i.e., involving high dimensional and sensitive settings, leading to less successfully-adapted DRL systems as well as more non-adaptable ones.

Researchers in software engineering in general, and in DRL in particular, are actively working on approaches to improve the self-adaptability of software systems in order to cope with ever-changing requirements throughout operation [ref]. We believe that our approach, \name{}, is in line with these current efforts and is a step further in assuring the DRL system's self-adaptability.\\

\begin{tcolorbox}[colback=blue!5,colframe=blue!40!black]
\textbf{Finding 2.} \name{} outperforms the vanilla CL in adapting a higher proportion of DRL systems to drifted environments, expanding the CL adaptability frontiers.
\end{tcolorbox}

\subsubsection{RQ3 (Performance): Are \name{}'s adapted systems more performant in terms of average reward than their CL counterparts?} \hfill

\noindent{\textbf{Motivation:}} The goal is to compare \name{} with the CL strategy in terms of the adapted system's performance on drifted environments. Predictive performance is 'the' requirement to fulfill for approving self-learning systems. Hence, assuring performance is an important phase in the adoption of any strategy involving self-learning systems (and DRL systems in particular).

\noindent{\textbf{Method:}} In this RQ, we consider the two following scenarios: (i) jointly adaptable environments, belonging to agent-environment pairs where CL and \name{} both succeeded in adapting the DRL system; (ii) jointly non-adaptable environments, belonging to agent-environment pairs where CL and \name{} both failed in adapting the DRL system. In these two scenarios, we average the rewards obtained by the adapted agent over the course of 100 consecutive episodes, using both alternative strategies. Then, we calculate \name{}'s average reward increase ratio, \%IR (Eq.~\ref{IR}), w.r.t the CL's average reward. Besides, the remaining scenarios, in which one strategy succeeds and the other fails, are irrelevant for reward comparison because the gap between them will be wide due to the failure of adaptation.

\begin{table}[]
    \caption{Comparison of Adapted DRL Agent Reward Increases Using Dr.DRL over CL.}
    \label{tab:reward}
    \centering
        \input{tables/reward.tex}
\end{table}

\noindent{\textbf{Results:}} The first part of Table \ref{tab:reward} (i.e., Rows 2–4) shows the reward increase ratio of \name{} compared to vanilla CL in jointly adaptable environments. \name{} achieves a similar average reward (no less than -1.2\%) compared to CL in 78\% of configurations. In the remaining 22\% of configurations, \name{} increases the average reward obtained by at least 10\%. To conclude, \name{} succeeds in preserving or improving the baseline average reward achieved by CL in jointly adapted environments, hence improving the performance of DRL systems.\\
The second part of Table \ref{tab:reward} (Rows 5-7) shows the reward increase ratio of \name{} compared to vanilla CL in jointly non-adaptable environments. As can be seen, \name{} was able to improve the average reward in 78\% of the configurations by up to 45\% of the increase ratio w.r.t CL's average reward. Hence, we highlight how \name{} achieves average rewards closer to the requirements compared to CL in the drifted environments that are still non-adaptable by both approaches.

\begin{tcolorbox}[colback=blue!5,colframe=blue!40!black]
\textbf{Finding 3:} \name{} was capable of achieving similar or even higher performances in adaptable environments, and it also earned higher performances in non-adaptable ones, showing how much closer \name{} was to meet the requirements than CL.
\end{tcolorbox}


==> preliminaries_backup.tex <==
This section contains a brief introduction to deep neural networks (DNNs), reinforcement learning (RL), continual learning and RL environmental drifts, as well as intentional forgetting.


\subsection{Deep Neural Networks}
A deep neural network (DNN) is an artificial neural network with a stack of multiple computational layers, hence the adjective `deep'. A DNN encapsulates a mapping function $y=f(x)$ that maps the input $x$ to its associated output $y$. As formulated below, the mapping function $f$ is a composite function of all the subfunctions $f(f_{l-1}; W_l, b_l)$, where $W_l$ and $b_l$ represent the learnable parameters, respectively, weights and biases.
\begin{footnotesize}
\begin{equation}
f(x ; W, b)=f_{L}\left(f_{L-1}\left(\ldots f_{1}\left(x ; W^{[1]}, b^{[1]}\right)\right) \ldots; W^{[L]}, b^{[L]}\right)
\end{equation}
\end{footnotesize}
Where $W = \{W^{[l]}, \forall \,l \in [1 , L ] \}$ and $b = \{b^{[l]}, \forall\, l \in [1, L]\}$. \\
DNNs learn their parameters using a backpropagation algorithm, which iteratively updates their parameters with the aim to reach an optimal set of parameters, producing a best-fitted DNN with low error rates. Backpropagation algorithm involves the following two alternative main steps, namely, forward pass and backward pass.

\textbf{Forward Pass.} A hidden layer $l$ performs a linear transformation $z^{[l]}$ of their inputs, i.e., the activations computed by its previous layer, then applies a non-linear activation function, $g$. Thus, the forward pass can be formulated as follows:
\begin{small}
\begin{equation}
\label{eq:act}
\begin{aligned}
&z^{[l]}=W^{[l]} a^{[l-1]}+b^{[l]} \\
&a^{[l]}=g\left(z^{[l]}\right) \\
\end{aligned}
\end{equation}
\end{small}

\textbf{Backward Pass.} As formulated in the below Equations, the backward pass involves computing the gradients of the loss, $\mathcal{L}$, with respect to the weighted-sum outputs of each layer, ${z}^{[l]}$, then with respect to the layer parameters, $W^{[l]}$ and ${b}^{[l]}$. Using the derivative chain rule, the gradients computed for a layer are leveraged to compute gradients in adjacent layers, inversely (from the input layer to the output layer).

\begin{small}
\begin{equation}
\label{eq:gradient}
\frac{\partial \mathcal{L}}{\partial {z}^{[l]}}=\left[{W}^{[l+1]}\right]^{\mathrm{T}} \cdot \frac{\partial \mathcal{L}}{\partial z^{[l+1]}} * g^{[l] \prime}\left(z^{[l]}\right)
\end{equation}
\end{small} 
\begin{small}
\begin{equation}
\frac{\partial \mathcal{L}}{\partial W^{[l]}}=\frac{\partial \mathcal{L}}{\partial {z}^{[l]}} \cdot\left[{a}^{[l-1]}\right]^{\mathrm{T}} \quad; \quad  \frac{\partial \mathcal{L}}{\partial {b}^{[l]}}=\frac{\partial \mathcal{L}}{\partial z^{[l]}}
\end{equation}
\end{small}
Therefore, the parameters are updated in the opposite direction of their gradients w.r.t the loss $\mathcal{L}$ using a learning rate $\eta$, as formulated below.
\begin{small}
\begin{equation}
W^{(i+1)}=W^{(i)}-\eta\: \frac{\partial \mathcal{L}}{\partial W^{[l]}} \quad; \quad b^{(i+1)}=b^{(i)}-\eta\: \frac{\partial \mathcal{L}}{\partial {b}^{[l]}}
\end{equation}
\end{small}

In several empirical studies aimed at demonstrating the interpretability of DNNs, it has been found that hyperactive neurons (i.e. neurons with high levels of activation) can provide beneficial learning patterns for DNNs [ref1, ref2]. In their work, Ma et al. [ref] identify hyperactive neurons and their combinations to depict the neurons responsible for major DNN behavior, while hypoactive neurons are attributed to minor DNN behavior. In our work, we build on these findings and rely on the definition of hyperactive and hypoactive neurons to identify the structural patterns of major and minor behaviors in the neural network.

\subsection{Reinforcement Learning}
Reinforcement Learning (RL)~\cite{sutton1998reinforcement} is a mathematical framework for experience-driven autonomous learning. RL aims to create fully autonomous agents that interact with their environments to learn optimum behaviors and improve over time. RL assumes that the agent's training goals can be quantified as the maximization of its cumulative obtained rewards (i.e., return) over its lifetime. To maximize a numerical reward, RL iteratively learns a policy, i.e., how to behave in each state of the environment, through trial-and-error interactions. Formally, the agent is given a state $s$ at each time-step $t$ of its interaction with the environment, and it decides which action to take based on that state. Those actions are determined by its on-learning policy, $\pi$, encoded as state-to-action mappings. Once an action is taken, the agent receives a reward and the environment moves to the next state. In our research, we consider episodic tasks that the agents must solve before their interaction with the environment ends according to certain conditions. Hence, the goal of our studied RL agent is to find the optimal policy, $\pi^*$, which maximizes the expected return at the end of episode. In terms of RL algorithms, there are several choices and configurations to consider. In the following, we describe the RL algorithms that we use in our experiments. First, we use deep reinforcement learning (DRL) that leverages deep learning (DL) to enable RL for complex, high-dimensional state and action spaces. Actually, DL models are non-linear function approximators that are trained to estimate quantities that depend on state and/or actions, e.g., a policy $\pi$ or an action-value function $Q$. Second, RL algorithms can use a model of the environment, i.e., simulation of environment behaviors given a state, an action, and a reward.  Model-based RL algorithms leverage a model of the environment that can be either available or learned; otherwise, they are named model-free. To avoid modeling biases and solve environments with complex dynamics, we decided to focus our study on model-free DRL algorithms. Model-free algorithms can be divided into the following three categories:\\
\textbf{Policy gradients.} The policy $\pi$ is represented by a neural network whose weights are updated by maximizing the expected return. This optimization is performed on-policy, meaning that each update is carried out with data (i.e., states, actions, and rewards) coming exclusively from the actual policy.\\
\textbf{Value-based.} The action-value function, $Q$, is represented by a neural network whose weights are updated based on the Bellman equation. This optimization is performed off-policy, meaning that it leverages data coming from any policy, not only from the actual policy. Based on a fitted $Q$ function, the policy is derived from choosing the action with the highest $Q$ value for all the states.\\
\textbf{Hybrid.} DRL algorithms belonging to this category use both policy gradients and value-based methods. One notable class of algorithms from this category is Actor-Critic algorithm which has two networks: Actor and Critic. The actor decides which action should be taken and critics inform the actor how good the action was and how it should adjust. The learning of the actor is based on the policy gradient approach, the critic evaluates the action produced by the actor by computing the value function.

\subsection{Environment Drift and Continual Learning}
% The term, environment drift, refers to a substantial change in the parameters of the environment that may affect the performance of trained agents. It corresponds to concept drift in supervised classification \cite{webb2016characterizing}, which refers to a change in feature-based probabilities of data, such as variations in objects' appearance or surrounding illumination. Indeed, a drifted environment provides the learner with new, unexpected data, i.e., the rewards associated to a certain state-action pair $(s, a)$ have been deviated. Although a drifted environment yields different rewards for a subset of state-action pairs, it should not be considered as a completely new environment. In fact, the original environment and its drifted counterpart share some regions of state-action space. However, in a completely new environment, the state-action space has no guaranteed connections with any previous environment. Hence, an agent should begin the learning process from scratch in a completely new environment because it requires replacement learning, whereas learning in a drift environment requires only further fine-tuning \cite{ring1994continual}, i.e., fusion of new information with the existing knowledge. This required fine-tuning is called the continual learning problem in deep learning \cite{hadsell2020embracing}, which investigates whether neural networks can acquire new knowledge incrementally. In spite of its success in several use cases, it has been shown that new knowledge may interfere with the existing one, which results in replacing it entirely. This failure of stability in the continual learning is called catastrophic forgetting \cite{french1999catastrophic}, in which new experience overwrites previous experience. Thus, the fundamental objective is to design a system that is plastic (i.e., adaptable) enough to continually incorporate new knowledge, but that, at the same time, remains stable and does not forget the acquired knowledge. 

Standard environment settings are often not representative of all possible contexts that RL agents will encounter for task fulfillment [refs]. The behavior of these environments is subject to changes, which can manifest as alterations in real deployment environments or shifts in the parameters of virtual environments \cite{wang2016novel, wang2019incremental}. These challenges, known as partial observability and non-stationarity [ref] in DRL literature, hinder productionizing DRL to real-world problems [refs]. For instance, recommender systems have no observations of the ever-changing mental state of the users and need to always heal their behavior accordingly. These changes in the production environment, called environment drift, may affect the performance of trained agents. The environment's behavioral changes become classified as environmental drifts when their severity/intensity is substantial, preventing the trained agent from achieving an average reward above a predefined threshold (i.e., the agent is no longer qualified). Although a drifted environment yields different rewards for a subset of state-action pairs, it should not be considered a completely new environment. In fact, the original environment and its drifted counterpart share some regions of state-action space. However, in a completely new environment, the state-action space has no guaranteed connections with any previous environment. Hence, an agent should begin the learning process from scratch in a completely new environment because it requires replacement learning, whereas learning in a drift environment requires healing by further fine-tuning \cite{ring1994continual}, i.e., the fusion of new information with the existing knowledge. This required fine-tuning is called the continual learning problem in deep learning \cite{hadsell2020embracing}, which investigates whether neural networks can acquire new knowledge incrementally. In spite of its success in several use cases, it has been shown that new knowledge may interfere with the existing one, which results in replacing it entirely. This failure of stability in continual learning is called catastrophic forgetting \cite{french1999catastrophic}, in which new experience overwrites previous experience. Thus, the fundamental objective is to design an advanced self-healing approach to improve the adaptability of DRL systems effectively and efficiently.

\subsection{Software Self-Healing and Intentional Forgetting}
More than ever, software systems must deal with change [refs]. Software should be able to perform under circumstances other than those for which it was intended. Continuous software availability requires considering fluctuations and shifts in production conditions as part of the development process. Software healing approaches [refs] have been explored to fix software system issues "in the field", as opposed to software repair solutions [refs], which are used "in-house" for bug-fixing operations. Indeed, healing approaches respond to software failures in production by making the appropriate adjustments, at runtime, to restore the system's normal behavior [refs]. When these adjustments are fully automated without human intervention, the approaches are called software self-healing [refs]. Software healing starts with the detection of misbehaving software that deviates from its intended function. Then, the healing operation involves the resolution of detected failures, or at least, mitigating their undesirable effects. Finally, a verification step ensures that the software system is restored properly. Otherwise, the healing step may be repeated (e.g., with a different healing operation) until the issue is fixed or no more actions are possible [refs]. DRL systems are data-driven and able to continuously adjust their internals to environmental shifts [ref]. Nevertheless, the continual learning of DRL systems can be less effective and more time-consuming as environmental drift becomes more severe. In this work, we aim to propose a novel advanced self-healing operation for DRL systems that leverages an intentional forgetting mechanism. 

Inspired by human cognition, intentional forgetting mechanisms are designed to improve decision-making by maintaining relevant knowledge [ref]. Indeed, researchers have employed intentional forgetting in computer science fields [ref] including cybersecurity [ref] and machine learning [ref]. In general, systems should be able to purposefully remove behaviors that lose relevance in relation to certain condition changes, either totally or partly [ref]. For instance, Authors [ref] propose a data selection technique with passive (removing obsolete data) and active (ignoring irrelevant data) during the DNN training. An example from the cybersecurity field is the self-defense techniques that erase leftover sensitive information from previous calculations to prevent potential attacks [ref]. This work is, to our knowledge, the first attempt to apply the concept of intentional forgetting to the DRL self-healing workflow.

%Software healing might or might not require human intervention. When the human is completely removed from the workflow, this approach is referred to as software self-healing [refs]. The demand for autonomous maintenance in today's software systems has prompted the establishment of several research disciplines with overlapping aims, including autonomic computing [refs], self-adaptive systems [refs], and self-healing systems [refs]. Research on self-healing systems, the focus of this work, has its roots in fault-tolerant and self-stabilizing systems research [refs]. Self-healing systems are systems that autonomously recover from an undesirable behavior, return to a normal one, and resume ordinary operation. These systems can withstand continuous availability (continuity) while being resilient to both deliberate, necessary adaptations and unexpected, random behavior. DRL is an innovative paradigm for building self-healing systems in the presence of environmental shifts [ref]. In this work, we aim to propose a novel advanced self-healing operation for DRL systems.

%In the course of human evolution, learning and forgetting have emerged as beneficial mechanisms for interacting with available information by adding/discarding new/unneeded knowledge to/from human memory. Psychologically speaking, humans deal with information explosion by forgetting knowledge selectively. Forgetting may be described as the inaccessibility of some previously learned knowledge. [ref]. It is an adaptive function to eliminate, replace, or rearrange outdated knowledge [ref]. For humans, forgetting is an intentional technique designed to facilitate decision-making by focusing on pertinent inputs [refs]. By adapting theories from human cognition, researchers are starting to employ forgetting (i.e., intentional forgetting) in software engineering [ref] in fields like cybersecurity [ref] and machine learning [ref]. In software systems, intentional forgetting is the capacity to enable knowledge to fade, i.e., to lose its relevance in relation to specific activities, either totally or partly [ref]. If software systems would preserve all learned and gained information this might lead to contradicting knowledge to perform required actions [ref]. Therefore, to accomplish certain activities based on gained knowledge, a knowledge base must be reliable (e.g., using an intentional forgetting mechanism).

%In cybersecurity, intentional forgetting is proposed to offer “forget patterns” to, e.g., delete leftover sensitive information and ensure cybersecurity assurance [ref]. Moreover, in machine learning, we are witnessing works like [ref] that propose a data selection technique with passive (removing obsolete data) and active (opting not to consider irrelevant data) forgetting for DNN training. Finally, the German national science foundation has lately launched the interdisciplinary priority research program "Intentional Forgetting in Organizations"[ref], supporting interdisciplinary initiatives in psychology, computer science, and business information systems. This project and the aforementioned study directions highlight the immense potential of intentional forgetting as an emerging research topic. This work is, to our knowledge, the first attempt to apply the concept of intentional forgetting in DRL.



